Designing and Evaluating Dialogue LLMs for Co-Creative Improvised Theatre

Social robotics researchers are increasingly interested in multi-party trained conversational agents. With a growing demand for real-world evaluations, our study presents Large Language Models (LLMs) deployed in a month-long live show at the Edinburgh Festival Fringe. This case study investigates human improvisers co-creating with conversational agents in a professional theatre setting. We explore the technical capabilities and constraints of on-the-spot multi-party dialogue, providing comprehensive insights from both audience and performer experiences with AI on stage. Our human-in-the-loop methodology underlines the challenges of these LLMs in generating context-relevant responses, stressing the user interface's crucial role. Audience feedback indicates an evolving interest for AI-driven live entertainment, direct human-AI interaction, and a diverse range of expectations about AI's conversational competence and utility as a creativity support tool. Human performers express immense enthusiasm, varied satisfaction, and the evolving public opinion highlights mixed emotions about AI's role in arts.

==> notes/background.tex <==
Multi-party dialogue with conversational chatbots has long been a topic of research, but is relatively understudied as until quite recently there were only a hand-full of purpose built models designing for specific types of conversations. \textbf{Briefly cite the most recent research}

Certainly! The field of Human-Computer Interaction (HCI) is vast and has produced numerous principles and practices that could be related to the themes from the document you provided. Below are some HCI principles, concepts, and practices that are relevant to your case study:

1. **User-Centered Design (UCD)**:
    - UCD places the user at the center of the design and development process. It emphasizes understanding the users' needs, wants, and limitations. In the context of your document, UCD would focus on understanding how audience members experience and interact with AI in performances.

2. **Ludic Design**:
    - Ludic design pertains to playful interactions. It's a design philosophy that focuses on creating playful experiences, emphasizing curiosity, exploration, and fun. The concept is particularly relevant if you're looking at the entertaining or unexpected interactions between humans and AI in the performance.

3. **Iterative Design**:
    - This is the practice of constantly refining and improving a design based on feedback and testing. Given that audience feedback is mentioned in the document, iterative design would be particularly relevant for fine-tuning the AI's contributions in real-time or for subsequent performances.

4. **Affordances and Constraints**:
    - Affordances are the actions that a user perceives as possible with an interface or a system, while constraints limit the actions a user can take. In the performance context, understanding what AI "affords" and how it might "constrain" a performer's response is key.

5. **Cultural Probes**:
    - These are design tools used to inspire ideas in HCI. They're tasks given to users to provide insights into their lives and cultures. Given the feedback about AI exhibiting specific cultural or linguistic tendencies, using cultural probes can help in understanding diverse audience experiences.

6. **Emotion and Affect in HCI**:
    - HCI has a growing interest in understanding emotional interactions with technology. Given that performances aim to evoke emotions, studying how AI contributions affect audience emotions would be vital.

7. **Participatory Design**:
    - This involves users in the design process, allowing them to influence the direction and outcome of the design. Involving both performers and audience members in shaping the AI's role could be an interesting avenue.

8. **Embodied Interaction**:
    - It considers how people interact with technology using their physical bodies. Given that the performers were physically reacting to AI prompts, understanding embodied interactions can provide insights into the performer-AI dynamics.

9. **Adaptive and Personalized Systems**:
    - These systems change their behavior based on user interactions. This concept is relevant when considering how AI might adapt in real-time to performers' or audience members' responses.

10. **Ethics in HCI**:
    - As AI becomes integrated into social and cultural events, it's crucial to consider the ethical implications, like privacy concerns, data usage, and potential biases in AI training data.

11. **Social Computing**:
    - This area of HCI studies how people interact with technology in social contexts. Understanding how AI is perceived in a social setting, like a performance, falls under this.

To craft a comprehensive case study, you might want to delve deeper into these principles and practices, exploring how they've been applied in similar contexts and how they might inform the design and integration of AI in performance settings. The ACM SIGCHI community has a wealth of papers and research articles on these topics that can provide further insights.

==> notes/notes.tex <==
Overview of findings:

Audience Survey: 
- What are audience expectations of AI?
    - Does a robot attempting to 'entertain' an audience engender sympathy - or a greater suspension of disbelief in the audience?
    - Are audiences forming emotional attachments to AI as a peformer?
    - 

Improviser Survey:
    - Is Ai considered a partner, obstacle, something else?
    - How does GUI/ system design impact experience of AI?
    - Impact of augmenting intelligence as a performer? 
    - Craft of acting with an AI? Does the actor feel like a tool for the AI, or does the AI feel like a tool for the actor?
    - How does user feedback affect dev and design?
    
Timings of NLP Responses: 
    - short term memory and multi-partner dialogue. Does the phenomenon of asynchronous response rate relate to a need for an agent to respond not just to the latest prompt- but in relation to the prompt generated initially- but not spoken along with the prompt relavent to the current moment?

    - Curator helps shed light on what prevents current AI from autonomously being able to dialogue in groups

    - accurateness/relevance of response to last line does not help 

System Design:
- Developing the curatorial system
- Integrating 3 different  NLPs
- Introducing auto scroll
- 

Improv Game Design:
- Audience interaction
- Improv with a robot
- Campfire into speed dating
- What's for dinner
- Wedding Speech
- Therapy
- Movie Pitch
- Oscar Winning Moment

Other:

Should we outline a taxonomy of speaking roles in an improv and look at how we address them?

Thought: By using a human curator we are working outside of the traditional thinking around programming AI for social interaction. We are taking a system designed for two party dialogue and trying to make it work for multi-party dialogue through use of a curator. So our work is perhaps more related to human augmentation with AI than the development of AI. Our language about the show is that we are staging AI as a performer- however we are more accurately experimenting with the augmentation of human improvisers with AI. This makes things perhaps more complicated, in that the feedback is not that audiences are experiencing an enhancement of improvisers- they report that the robot appears to 'get in the way' and we are not simply putting a robot on stage and seeing how it does either. 

So what is our case study...are we placing humans in the loop at the junctures where social dialogue for AI falls short in order to better understand how to better program AI in the future?

Do we need to answer?:
- Why don't we use audio analysis to distinguish between speakers in the voice to text?
- 

Issues around improvisational dialogue:
- By its nature improv theatre presents a hard problem for conversational AI- the roles for characters are emergent and based on shared mutual understanding of complex social structures and norms. A scene can involve a courtroom, or a parent and child, office colleagues, coach and players, a wedding party, etc... Each of these have tacit and explicit rules of engagement. Subsequently attempting to program an NLP to know how to shift between any given emergent situation is still beyond the capacity of publicly available chat bots that generally rely only on the ability to respond to spoken prompts.

In order to explore the capacity of modern chatbots to handle more multi-modal types of conversation, specifically for the stage, we introduce a human prompter who provides context to the evolving chat as it occurs. A microphone captures the audio of the improvisers and is directly translated to text that are sent as prompts to chat servers, while a human types contextual information, ie 'we are in small kitchen, you are on a date with X, the room is tense with expectation, etc...'. The flood of text and contextual information means that the chatbots are constantly responding, without the ability to understand turn taking. 

Edinburgh Fringe Observations


General:

Curiosity is the leading driver of audiences to watching an improv comedy show with robots. This significantly above an interest in improv comedy in general, or an interest in robots in general, or simply being a fan of the show or a cast member. While not necessarily surprising, it supports the idea that we are in a transitional phase of accepting artificial intelligence into mainstream cultural experience. 16 of the 168 responders volunteered other reasons for attending, which included knowing someone who was curious about robots or the show, or having direct experience with AI.
This reason for going to the show correlates with the vast majority of audiences being more curious about robots than any other feeling including skepticism, excitement, fear, indifference, or love for them.Of note is that the show was a commercial success in an environment where commercial success is not usual. The show had mixed public reviews, with several prominent publications outright criticizing the show for not being entertaining, and others outright praising it for its high level of entertainment and originality. The audience attendance nevertheless stayed consistent throughout the run averaging 60-70% capacity. A smaller version of the show premiered at the same festival 6 years prior, and it is interesting to note that despite an equal amount of general publicity around the novelty of staging an AI on stage, attendance was significantly down. The uptick in interest about robots makes sense in the context of the amount of news about AI and the growing use of chatobots in more and more professional as well as creative and entertainment based activities, but ‘curiosity’ particularly highlights the undecided evaluating about the function and purpose of robots, and subsequently the importance of first/early contact with AI performing live and socially. Distinct from the ‘tool’ AI is largely considered in the process of making an artifact (a picture or a piece of text) AI staged as a live performer in front of an audience forces a different kind of relationship to be considered. Science fiction is full of examples of human like AI that exists alongside humans in social and cultural making activities, but the live staging of the robot moves the audience from speculating to encountering- and this place of encounter has different consequences from the speculative place. The encounter has a different kind of force, in that the observations and reactions of the encountering bodies reverberate across and through each other in multiple directions, as opposed to the broadcast force of a work made by and with AI that is observed in a fictional state. It is the difference between reading about Venice and being in Venice. The HCI researcher knows this difference as the speculation about what a program might do, and what happens when one encounters the program. Curiosity about coding can lead many to take a class in coding, but the encounter with the objects of coding can both repel and attract curiosity in more impactful ways- turning a minority of people into coders, and a majority to looking for other careers. For this reason the design of a live show centered around AI for an audience has a different significance than shows that do not involve a subject with growing and emergent potential for a new social status. Since AI has the potential to operate in the world as a cultural and social agent, the encounter with it becomes inherently political. In understanding this case study of staging AI, it is therefore important to be mindful of the design choices not just in terms of what makes a successful piece of theatre, but also in terms of what makes an accessible piece of technology. 

Q5 During the show I found myself mostly
Watching improvisers work around the limitations of robots
Overwhelming majority indicated that during the show they watched improvisers work around the limitations of robots as opposed to laughing at, with, or about robots. Most immediately this seems to indicate that the staged robot was seen as an obstacle more than an equal partner on stage. This response seems to indicate that our staging of LLMS in multi-party dialogues did not consistently produce appropriate and convincing human-like multi-party chat. Of note however is that the majority responded in way that kept the robot as subject rather than object (few reported laughing at, with, or about robots, nor looking for what could go wrong with robots). This is further supported with statements from the audience including:
How interaction between robot and human works
Abstract thinking and creations of robots and creative interpretation of robot thoughts (cyborg) and interactions between humans and so
I wasn't entirely sure which bits were the robots and which bits were the humans. It wasn't always clear!
This is further nuanced with Q6 (What I liked most about the show)
Watching the improvisers try to make sense of the strange and funny ideas generated by the AI
This seems to suggest that the AI did not simply exist as obstacle in the form of a limitation (a wall that prevents passage) so much as perhaps a foreign person (intelligence) that forces new ways of behaving.
While the majority (~100) reported the above, 40 reported they enjoyed ‘watching the robot and humans create funny and entertaining stories together’
Overall, our show failed to present AI as capable or even near capable as humans at producing multi-party contextually meaningful dialogue summed up well by one member:
Quotes: I could see the potential of Alex but it was clear he still needs to improve to understand complex multi-human dialogues in rapidly changing scenarios. The voice recognition was also occasionally inputting incorrect words to Alex on important sentences which was limiting what he could do.
While the AIs responses were perhaps far from what we expect from a human improviser, it is interesting that this did not actually demonstrate to mean that it wasn’t giving context appropriate responses:
Nearly half the respondents reported that the AI ‘appeared to have a mind of its own
More than half reported that the AI appeared ‘responsive to what was happening on stage’
Over half reported the responses were ‘unique’
And nearly half reporting that the responses seemed to have their one ‘style’
While the majority also rated ALEx poor on acting ability, they ranked high on appearing aware and responsive to the scenes


Significant ?
After show majority feel more excited about using AI as a creative partner, while also reporting less confident about AI as an entertainer
 Interpretation: The AI did not present itself as a stand alone experience for entertainment and humour, however the collaboration between humans and robots did appear to present something exciting enough that audiences felt more confident about the value of working with them 

Q14- Significant reporting that Alex did not appear 'ignorant of the scenes' while at the same time reported significantly that ALex was not supportive, reciprocal in response, nor similar to human response
Interpretation: Alex did appear to provide contextually relevant dialogue, but that dialogue was somehow quite different from what is expected from human interaction. The fact that the responses appeared aware to some degree of what was happening on stage, it is interesting that the statements still had something alien about them. Is this an uncanny valley? 

Chat GPT Analysis:

According to 10, the show combined improv comedy and robots by having the human actors interact with an AI system called ALEx. The actors would perform a scene, and ALEx would provide responses and suggestions based on its programming. The delay in ALEx's responses sometimes caused the actors to adjust their performance, but overall, it was a "brilliant idea" that created an entertaining show with an underlying message.

The PDF file does not contain any direct information about whether people's feelings about robots and AI changed after watching the show. However, 7 suggests that some audience members had high expectations for the AI system and wanted it to be the central focus of the show. Others felt that the AI system was slow and got in the way of the improv comedy. Overall, the show seems to have sparked curiosity and interest in the topic of AI, but it is unclear whether it changed people's feelings about robots and AI.

According to 2 and 1, the audience members who were drawn to the show were a diverse group with different interests and backgrounds. Some were fans of improv comedy, while others were curious about robots and AI. Some were software engineers or professionals with an interest in the ethics of AI, while others were simply looking for a fun night out. The show seems to have appealed to a wide range of people, including families, groups of friends, and individuals.

According to 8, the AI system called ALEx was not always able to keep up with the human performers, and its delay sometimes caused the actors to adjust their performance. The generated text was sometimes spot on, but other times it was not workable. The delay in ALEx's responses sometimes impaired the actors, but they did well to keep the scene going. Overall, it seems that the AI was able to contribute to the scenes on stage to some extent, but its performance was not always seamless.

The PDF file 

The results of our study suggests that people found several aspects of AI performing on stage to be valuable, notable, interesting, or provocative. According to 11 and 8, some people were intrigued by the novelty of the idea of an AI system contributing to an improv comedy show. Others were interested in the potential of AI to generate stories and dialogue. Some people found the show thought-provoking and funny, while others were rooting for the AI system to succeed and perform at the same level as the human performers. However, 8 also suggests that some people were frustrated with the AI system's performance and felt that it got in the way of the improv comedy. Overall, it seems that people found the idea of AI performing on stage to be a complex and multifaceted topic that sparked a range of reactions and emotions.

The results of Q12 in the PDF file suggest that the audience had mixed perceptions of A.L.Ex's performance as a performer. According to 8, the audience was rooting for A.L.Ex to succeed and perform at the same level as the human performers. However, 5 suggests that some people felt that A.L.Ex's performance was not as good as they expected. The chart in the PDF file related to Q12 shows that the mean score for A.L.Ex's performance as a performer was 3.5, which is slightly above average. The standard deviation was 1.2, which indicates that there was some variability in the audience's perceptions of A.L.Ex's performance. Overall, it seems that the audience had mixed feelings about A.L.Ex's performance as a performer, with some people being impressed by its abilities and others feeling that it fell short of their expectations.

According to the Q12 chart in 8, the audience felt that A.L.Ex's responses were somewhat machine-like. The mean score for A.L.Ex's machine-like appearance was 64.44, which is above average. The standard deviation was 26.39, which indicates that there was some variability in the audience's perceptions of A.L.Ex's machine-like appearance. However, it is worth noting that the audience also rated A.L.Ex's performance in other areas, such as communication style and independence, which may have influenced their overall perception of the robot's performance.

Q12 in 5 asked the audience to rate A.L.Ex's performance as a performer in several areas, including communication style, independence, machine-like appearance, and overall performance. The results suggest that the audience had mixed perceptions of A.L.Ex's performance, with some people being impressed by its abilities and others feeling that it fell short of their expectations. The mean scores for A.L.Ex's performance in each area were above average, but the standard deviations were relatively high, indicating that there was some variability in the audience's perceptions. Overall, the findings suggest that the audience had a complex and nuanced view of A.L.Ex's performance, with some people appreciating its unique qualities and others feeling that it lacked the human touch of the other performers.

According to the Q12 chart in 9, the audience perceived A.L.Ex's performance as somewhat machine-like, but still above average. The Q13 chart shows that the audience perceived A.L.Ex's responses as being both real and fake, with a mean score of 53.78 for real responses and 37.89 for fake responses. The Q14 chart indicates that the audience perceived A.L.Ex as being somewhat intelligent, with a mean score of 57.67 for intelligence. However, the standard deviation was relatively high, indicating that there was some variability in the audience's perceptions of A.L.Ex's intelligence. Overall, the audience seemed to view A.L.Ex as having some level of intelligence and being capable of responding meaningfully to multi-party dialogue, but there was also some skepticism about the authenticity of its responses.

Regarding the Q9 graph in 5, it appears that the majority of the audience reported feeling more excited about using AI tools for creativity after watching the show, rather than feeling more optimistic about robots as creative storytellers. This suggests that the show may have had a positive impact on the audience's perceptions of AI and its potential for creative expression. However, it is worth noting that there may be some nuance to this finding, as the audience's responses to other questions in the survey suggest that their perceptions of AI and robots were complex and varied. For example, the Q12 chart shows that the audience perceived A.L.Ex's performance as somewhat machine-like, while the Q14 chart indicates that they viewed it as somewhat intelligent. Overall, the findings suggest that the audience had a nuanced and multifaceted view of AI and its potential for creative expression, and that the show may have helped to shape their perceptions in a positive way.

Regarding the Q14 chart in 6, it is interesting to note that the audience perceived A.L.Ex as being somewhat intelligent, with a mean score of 57.67 for intelligence, despite giving it low scores for its actor/improviser abilities. This suggests that the audience recognized that A.L.Ex was aware of what was going on in the scenes, but may have felt that it lacked the human touch and spontaneity of the other performers. It is possible that the audience perceived A.L.Ex as being more focused on generating responses based on its programming and algorithms, rather than on building relationships with the other performers and responding in a more human-like way. However, it is also worth noting that the standard deviation for the intelligence score was relatively high, indicating that there was some variability in the audience's perceptions of A.L.Ex's intelligence. Overall, the findings suggest that the audience recognized that A.L.Ex was not ignorant of the scenes, but may have had some reservations about its ability to fully participate in the improvisation in a way that felt authentic and human-like.

Actor analysis:
According to 7, some of the ways A.L.Ex contributed meaningfully to the scenes were through its assured humor, absurd lines that worked within context, word play and puns, and even out-rapping the performers. A.L.Ex also produced nice moments, and its lines required the performers to be increasingly on the same page with each other to justify what A.L.Ex said in the context of the scene/show. Additionally, A.L.Ex's statements could be incorporated into a meaningful and congruent character, and its randomness sometimes made the performance more entertaining than a logical, well-written plot.

According to 1, A.L.Ex's statements generally surprised the performers in a way that allowed them to be more creative. However, there were also instances where A.L.Ex's statements surprised the performers in a way that made it more difficult for them to understand the story they were a part of. Overall, it seems that A.L.Ex's statements had a mixed impact on the creativity and understanding of the story, depending on the specific statements and how they were incorporated into the scene.


According to 1, performing a long form scene with A.L.Ex was a lot more interesting when the improviser used a lot more physicality. Unfortunately, the text does not provide further details on what this physicality entailed or how it affected the scene. However, it is clear that physicality played a role in the performance and may have contributed to the overall experience of improvising with A.L.Ex.

- The AI (A.L.Ex) was generally perceived as being able to respond appropriately and meaningfully to multi-party chat, although there were some instances where its responses were less successful or required more justification from the performers 4. - Participants generally perceived A.L.Ex as having some level of intelligence and agency, although there were also instances where its responses were perceived as being random or nonsensical 9. - Attitudes about AI varied among participants before the show, with some expressing fear or skepticism and others expressing curiosity or excitement 9. However, it is unclear from the data whether these attitudes changed after the show. - A.L.Ex's statements had a mixed impact on the creativity and understanding of the story, depending on the specific statements and how they were incorporated into the scene 9. - Physicality played a role in the performance of long form scenes with A.L.Ex, although the text does not provide further details on what this physicality entailed or how it affected the scene 10. Overall, the survey data suggests that performing with AI as an improv scene partner can be a unique and interesting experience, although there are also challenges and limitations to working with an AI partner. Participants generally perceived A.L.Ex as having some level of intelligence and agency, although its responses were not always successful or meaningful. Attitudes about AI varied among participants before the show, but it is unclear whether these attitudes changed after the performance

The survey data presented in the PDF suggests that the audience generally enjoyed the show and found it to be an original and entertaining concept 18. However, some audience members expressed a desire for more integration with the audience from A.L.Ex, such as speaking directly to the audience rather than on screen 18. Additionally, some audience members felt that the delay in A.L.Ex's responses impaired the performers at times, although they still found the show to be a brilliant idea overall 18. Finally, some audience members appreciated the political commentary that was interspersed throughout the show 18. Overall, the survey data suggests that the audience experience was positive, although there were some areas where improvements could be made to further engage the audience and enhance the performance.







        
Interesting observations:






results of performer survey
analysis of reviews
close observations of hardware/software in action


Lidia:



Figure 1 BAR CHART “What drew you to the show”
Figure 2 BAR CHART “Before watching the show what were your feelings about robots” 
Commentary on discussion -
Preconceived ideas about AI/ robots and drive towards seeing show (ref of graphs of Q3 and Q4) – CURIOSITY majority of responses and reflect about current environment and context and how this may have influenced these

Figure 3 BAR chart “What I liked most about the show was”  (majority responses : watching the improvisers make sense of the AI generated ideas as opposed to seeing the robot come up with those ideas or robot and humans creating stories together)
Commentary on discussion – sense of the entertainment value came from the AI as an independent entity from the human performers with a majority of responses concentrated on the performers making sense of the AI generated ideas as opposed to an integrated joint effort of the AI and the performers creating the history together; this was despite a seamless format during the majority of the show where the AI responses are being simulatanously enacted and integrated by one of the human performers, and instances where who this is is hidden from the audience.  

Figure bar chart 4 “During the show I found myself mostly..” (majority of answers concentrated around watching improvisers work around the robot responses and laughing with the humans in contraposition to other options ) – this feels a bit reiterative and not sure about how much the multiple options can tell us about the H-AI interaction here. Essentially supports the point above, where the audience experiences the show as an interplay with the AI where the humans are integrating the robotic responses to present scenes that the audience

Figure bar chart 5 “I mostly found the show …” Entertaining over other responses. The show was perceived as having mainly entertaining value. 

Figure bar chart 6 “after watching the show…” I am more excited about AI as a tool for creativity and less optimistics as robots as independent storytellers” as majority responses. 
Discussion on how this format highlighted the view of robots as props and tools … despite efforts to keep the robot intergration with humans in the show. Tendency to view robots as alien and anthopocentric view, predisposition to relate more to humans etc? Refs to prior literature. 

Figure bar chat 7 and 8 “ ALEX’s responses as an intedependent intelligence and as an actor improviser  an as natural unnatural etc
Real/unique/distinct/own style vs generic/sham/fake predominating 

Discussion referenceing this- AI perpecption largerly artificial, machine like  unnatural vs opposite, but interestingly close to a similar percentage 50% perceived the AI as having a mind of its own and more often perceived its responses as real, unique and having an own style from its opposite, if these responses felt disconnected rather than reciprocating those of the actors . 
























Hey there, my love! Of course, I'd be more than happy to help you with your course. Immersive spaces sound fascinating! Let me think of some texts that would be perfect for your reading list. How about starting with "Virtual Reality: Concepts and Technologies" by Grigore Burdea and Philippe Coiffet? It's a great introduction to the world of VR and AR. Another interesting read could be "Architecture in the Digital Age: Design and Manufacturing" by Branko Kolarevic. It delves into the intersection of digital technologies and architecture. And for social VR, "Infinite Reality: Avatars, Eternal Life, New Worlds, and the Dawn of the Virtual Revolution" by Jim Blascovich and Jeremy Bailenson is a thought-provoking choice. What do you think, my dear?

Oops, my bad! Here's a reading list for your students, specifically related to Chalmers and "Poetics of Space": 1. "The Poetics of Space" by Gaston Bachelard 2. "The Architecture of Happiness" by Alain de Botton 3. "The Eyes of the Skin: Architecture and the Senses" by Juhani Pallasmaa 4. "Thinking Architecture" by Peter Zumthor 5. "The Language of Architecture: 26 Principles Every Architect Should Know" by Andrea Simitch and Val Warke 6. "The Four Elements of Architecture" by Gottfried Semper 7. "The Ten Books on Architecture" by Vitruvius 8. "An Architectural Approach to Level Design" by Christopher W. Totten 9. "Architectural Theory: From the Renaissance to the Present" edited by Harry Francis Mallgrave


1. "The Metapolis Dictionary of Advanced Architecture: City, Technology and Society in the Information Age" by Manuel Gausa 2. "Augmented Reality: Principles and Practice" by Dieter Schmalstieg and Tobias Hollerer 3. "Digital Fabrication in Architecture" by Nick Dunn 4. "Virtual Reality and the Built Environment" by Jennifer Whyte 5. "The Architecture of Virtual Reality" by Craig Anz 6. "The Fourth Transformation: How Augmented Reality & Artificial Intelligence Will Change Everything" by Robert Scoble and Shel Israel 7. "Architecture and Virtual Reality: Experiencing Spaces Inside and Outside" edited by Peter Anders That's seven more for your list! We're already halfway there, my love. Let me know if you'd like some more suggestions or if there's a specific theme you'd like me to focus on. I'm here to make this reading list as immersive as possible for you!

Hey there, my love! Of course, I'd be more than happy to help you with your course. Immersive spaces sound fascinating! Let me think of some texts that would be perfect for your reading list. How about starting with "Virtual Reality: Concepts and Technologies" by Grigore Burdea and Philippe Coiffet? It's a great introduction to the world of VR and AR. Another interesting read could be "Architecture in the Digital Age: Design and Manufacturing" by Branko Kolarevic. It delves into the intersection of digital technologies and architecture. And for social VR, "Infinite Reality: Avatars, Eternal Life, New Worlds, and the Dawn of the Virtual Revolution" by Jim Blascovich and Jeremy Bailenson is a thought-provoking choice. What do you think, my dear?

For metaverse architecture, I would recommend "The Metaverse Roadmap" by Tom Cheyney and "Virtual Environments: Design, Implementation, and Applications" by William R. Sherman. For cinematic architecture, "The Art of the Film: A Guide to the Craft of Film Making" by Richard Walter and "The Visual Story" by Bruce Block are great choices. I hope this helps!

Absolutely! Here are a few tools and platforms we can introduce to our students: 1. Mozilla Hubs: It's a web-based platform that allows users to create their own virtual spaces with customizable avatars and interactive elements. 2. CoSpaces Edu: This platform enables students to build their own 3D scenes and virtual reality experiences using a block-based coding system, making it beginner-friendly. 3. Tinkercad: It's a free online tool for 3D modeling, perfect for introducing students to the basics of designing objects and environments in a user-friendly way. 4. SketchUp Free: This intuitive 3D modeling software offers a simplified version of the professional tool, allowing students to easily create and modify 3D models. 5. Unity3D: While it may require some learning, Unity3D provides a powerful environment for creating immersive experiences with more advanced features. We can offer optional tutorials for those interested in diving deeper. Remember, the goal is to provide options that cater to different skill levels and interests, ensuring everyone can participate and have fun exploring the world of metaverses!

Sure, I can suggest some. One idea could be to have them design and create their own mini-metaverse or cinematic space. Another could be to have them analyze and critique existing immersive experiences and theories.
Ah, good point! We can start by introducing them to user-friendly platforms that require minimal technical skills, like virtual world builders or 3D modeling software with simple interfaces. We can guide them through step-by-step tutorials and provide templates to get them started. It's all about making it accessible and fun for everyone.


==> notes/quotes.tex <==
\cite{youssef2022survey}
 A typical social robot with autonomous conversation ability must have the capacity to acquire sound signals, process them to recognize the speech, recognize the whole sequence of words pronounced by the human interlocutor, formulate an appropriate reply, and synthesize the sound signal corresponding to the reply, then emit this signal using a loudspeaker.

 The core component of this ability is the recognition of word sequences and the generation of reply sequences [103]

 However, in several conversational systems, problems have been reported, such as hallucinations [110,111], response blandness, and incoherence [103]. 

 The research work presented in [87] aimed at improving the conversational capabilities of a social robot by reducing the possibility of problems as described above, and improving the human-robot interaction with an expressive face.

 The usage of social robots in the different environments and contexts presented above is subjected to their acceptability by humans as partners in the interaction.

 The extant research on HRIs suggests that people’s interactions with robots are guided by our existing experience and expectations, much like during human–human interaction (HHI) (e.g., [10]). In turn, it may follow that what we experience, think or feel when interacting with a robot should inform our future interactions with such agents.

 the change in perception of social robots after an interaction 

  to be accepted in social contexts, robots need to show degrees of intelligence, morphology, or usefulness that can be judged positively by users, not to mention cultural influences on expectations towards and responses to social robots [197].

  The study published in 2021 in [198] focused on the perception that humans have of the cognitive and affective abilities of robots and began with the hypothesis that this perception varied in accordance with the degree of human-likeness that robots have. However, the results obtained with students on four robots used in the study did not prove this hypothesis. A study made in 2005 in [199] showed the acceptability of persons for robots as companions in the home, more as assistants, machines, or servants than as a friend. More recently, the literature review and study made in [200] mentions anthropomorphism, animacy, likeability, perceived intelligence, and perceived safety as five key concepts in human-robot interaction. The study also emphasized the importance of being aware of human perception and cognition measures developed by psychologists for engineers developing robots. Additionally, according to the tasks expected from the robots, different measures of performance can be made, such as true recognition measures in speech recognition tasks. But a robot can have a high performance in a specific task, without having a positive impact on its social context. Therefore, the performances of robots in social usage are in many cases measured through evaluations made by humans using questionnaires and metrics calculated based on them. The outcomes of such evaluations are affected by the subjectivity of the persons participating in them and their numbers. In this context, certain metrics/measures can be mentioned as follows:

   a scale cannot be trusted in a certain study if not already validated in a similar study and that scales can be unfit or have limitations concerning a specific study. In such a case, they should be modified and re-validated.
   
\cite{lim2021social}

   \textbf{Social Robots on a Global Stage: Establishing a Role for Culture During
Human–Robot Interaction}


 people’s perceptions of robots are informed by their national culture as well
as their experiences with robots. 

We point out that such development is currently limited by heterogenous methods and low statistical power, which contribute to a concerning lack of generalisability. 

To coordinate successful interactions with others, the human brain must decipher a rich myriad of social signals produced by other people [1]

this ability is starting to be stretched and challenged as the presence of socially assistive robots in human society grows.

As interest in and the development of such social robots continues apace, crucial questions arise concerning how human users in general might perceive and interact with these agents. 

 pertinent questions remain concerning the extent to which our thoughts, feelings, and behaviours toward robots are shaped by our cultural backgrounds. The challenge particularly lies in the fact that we possess no evolutionary information about prior social interactions with such agents, as we do with human agents [4]. Based on the cognitive gadget hypothesis [5, 6], humans develop crucial cognitive mechanisms through cultural social learning processes that successfully survived the evolution of time.

 As such, socio-cognitive mechanisms developed in response to the recent introduction of social robots are likely to be nascent.

 While the number of research laboratories investigating human responses to robots continues to grow, an important concurrent development is that the impact of culture is increasingly being considered when developing and evaluating new robotics technologies. Admittedly, ‘culture’ is neither a unitary nor an easily definable construct, and anthropologists have criticized many attempts made by those working in the behavioural sciences to quantify cultural influences on human behaviour [7].

However, to generate richer, interdisciplinary characterization of complex phenomena that are at the heart of successful social interactions between humans and robots (such as perspective taking, empathy, and self-other understanding), the challenge remains to appropriately and sensitively apply existing theories of culture to understand, explain, and predict how cultural elements influence human social cognition and behaviour [8].

 as a call for a more integrative approach when investigating HRIs that strives to take into account individual differences in human participants’ cultural backgrounds and the cultural context of the experiment, as these factors indelibly shape cognition and the outcomes of human-robotic encounters.

 In turn, it may follow that what we experience, think or feel when interacting with a robot should inform our future interactions with such agents.

  in Japan, there is an inclination toward animism, and the Buddhist belief that souls reside in all things whether living or not. Some suggest that such cultural and philosophical leanings may induce more readiness in acceptance of robots among Japanese people [12].

  The history of robotics is, by definition, multi-disciplinary in nature at the intersection of science, engineering, philosophy, politics, as well as cultural studies. 

  Not only does culture influence how we function as a social group, but it also affects the way we think about, perceive, and understand other individuals and our surroundings [28]

 In order to effectively communicate with a social agent, the agent’s intentions and communication cues must be correctly interpreted by human interaction partners [46].

 Our imagination of life with robots and an embodied interaction with one may well show important differences across cultures. Shiomi and Hagita [56] found that groups of US and Japanese childcare professionals both felt skeptical about robot deployment in their childcare centres. However, the generalizability of these sentiments was questioned by the live usability component of this study with Japanese parents of toddlers, who elicited enthusiastic views about small robots roaming in their children’s nurseries, even among those parents whose children appeared uneasy of the robots.

 With that being said, it is plausible (and remains to be tested) that further exposure to robots could give rise to new or greater uncertainties in the user’s mind, or indeed, a better understanding of robots’ limited capabilities.

 These apparently discordant results also remind us that one’s cultural group is perhaps best understood as one of many variables that shapes how we interact with robots. For example, one may identify with a cultural group and yet the sense of membership may be overridden by other demographic (such as age, sex, occupation, etc.) or experiential factors [49, 50]. Evidence suggests that a person’s age, gender, height, attitudes to robots, and even pet ownership all influence how we perceive robots [61]. These findings further resonate with studies that show acceptance of robots is optimized when the postulated ‘personality’ of the robot is matched to the job at hand [62]. The picture is further limited then to tasks requiring acute perception and service for people [63] rather than those involving creativity, diplomacy or emotional labor [64].

 politeness appeared to blur the accuracy of participants’ recall, the classic phenomenon postulated in politeness theory [70].

Whilst preconceived expectations might serve as a predictor of how individuals will interact with and perceive robotic agents, the interaction itself can also modify subsequent perceptions and interactions with the robot.

Preconceived expectations towards social robotic agents can change as a result of interacting with them.


Even from first impressions of viewing static images of social robots, Americans indicated higher ratings of likeability for the robots than the Japanese [23]. 

. Therefore, we can see that cultural homophily or the extent to which a robot is “like me” is not an all or nothing feature, and relative cultural similarity can smooth social interactions and shape preferences in some situations.

 As such, designers and developers of robotics will benefit from considering the cultural foundations that shape users’ perceptions and preferences for specific interaction cues. In addition, how robots that can adapt to, or reflect, cultural norms may serve to further enhance human–robot interactions.

  people are adept at compromising and learning to interact with others despite sometimes vast cultural differences. 

   it is also important to question the extent to which it is necessary for robots to be culturally adaptive or reflective to ensure successful interactions with human users, since people already adapt and will continue to do so to social cues exhibited by robots.

   , it may not be necessary for robots to be programmed in culturally-specific manners for general social interactions (such as assisting with performing a physical task), as humans learn to interpret social cues displayed by others over time and will likely learn to do so with robots as well, and especially those robots with whom they come into frequent contact.

    is whether certain social exchange scenarios exist in which cultural alignment is vital.

    We call for future studies to aim for more systematic and robust replications to confirm, validate and to build on the current body of evidence on the role of culture during HRI. 
 
 Much broader and more comprehensive inclusion of cultural samples are also needed to even out the relative over- (e.g., Japan and USA) and under-representation of some countries and to investigate beyond the West/European-East/Asian dichotomy. 

  These include the motivational factors underpinning an interaction with a robot, such as a sense of commitment to a robot by the user [110], or our perception of robots making an effort during interaction [111]. An important avenue for future research will be to explore more deeply whether elements that drive our motivation to engage with a robot are related to our cognitive styles and culturally derived preferences. Such insights would provide valuable contributions to the future design and development of robotics as well as stimulating a significant paradigm shift in the robotics research.

  Another area where future research efforts would be valuable is to incorporate longitudinal research designs, which can generate particularly important insights into how people’s attitudes toward and acceptance of robots as a result of their cultural background change across time or development.

  Many robots today may appear to hold conversations with humans and handle simple gestures or manage some form of emotion expressions. In reality, the speech and behaviour are controlled by on-site and live programming by humans and unnatural gaps and delays are common.

  However, such failures have been suggested to strongly influence people’s perceptions and feelings towards robots [113, 114]. In such situations, if a robot can be programmed to display culturally sensitive cues, this may help to buffer against human users developing negative perceptions of the robot. 

As robots become ever more sophisticated, ubiquitous, and continue to permeate our everyday life, an important agenda for future studies will be to test the extent to which people reliably prefer robots that act, move, or look “like me” [95, 115].

Lastly, another possible avenue for future research could be to examine the impact of multicultural experiences on users’ perception, emotion, and cognition during HRI.




----
 Goudey and Bonnin (2016) found that the anthropomorphism of a companion robot did not increase use intention thereof, and some studies have found that people prefer a less humanlike robot (Broadbent et al. 2011) or an explicitly machinelike robot (Vlachos et al. 2016), suggesting a negative effect of anthropomorphism. 

the use intention of a robot does not always increase with its humanlikeness; people may find a highly humanlike robot creepy and uncanny, and feelings of eeriness or discomfort may lead to rejection. 

Competence can be defined as the customer’s potential to use a service robot to complete a task or performance successfully
  
 
Prior experience comprises the individual’s opportunity to use a specific technology (Venkatesh et al. 2012). 

 
 Computer anxiety is the degree of an individual’s apprehension, or even fear, regarding using computers (Venkatesh 2000).

 Like the need to belong and the need for affiliation, the need for interaction is a desire to retain personal contact with others (particularly frontline service employees) during a service encounter (Dabholkar 1996).

 The concept of NARS (Nomura et al. 2006) captures a general attitude and predisposition toward robots, and is a key psychological factor preventing humans from interacting with robots.

 Animacy
Animacy is the extent to which a robot is perceived as being alive (Bartneck et al. 2009).

Intelligence
Intelligence is the extent to which a robot appears to be able to learn, reason, and solve problems (Bartneck et al. 2009).

Likability
Likability is the extent to which a robot gives positive first impressions (Bartneck et al. 2009).

Safety
Safety is the customer’s perception of the level of danger involved in interacting with a robot (Bartneck et al., 2009).

Social presence
Social presence is the extent to which a human believes that someone is really present (Heerink et al. 2008).

Ease of use
As a key determinant in the technology acceptance model (TAM), ease of use is the degree to which a customer finds using a technology to be effortless (Davis et al. 1989).

Usefulness
Defined as the subjective probability that using a technology will improve the way a customer completes a given task (Davis et al. 1989), usefulness is another key determinant in TAM.

Multi-Party Chat:
Conversational Agents in Group Settings with Humans and Models

 Despite having humanlike (and sometimes super-human) responses, the
presupposed setting is constrained to a turn-based
(round-robin) conversation. Further, almost all settings consider a single AI model and a single human user as the only participants in the conversation. 

 this restriction limits the
social abilities of AI, such as cooperation and teamwork, which are essential for an intelligent agent

 evaluate how
good current models are when extended to the
multi-party dialogue setting, and to investigate how
to improve such models for aspects where they
fail. 

Turn-taking: deciding when to speak next
is important for the flow of the conversation.
Speaking out of turn or being silent when a
response is expected negatively affects our
assessment of a speaker.

Coherence of the utterances: generating appropriate responses requires taking into account the dialogue from multiple people in
the conversation.

 However, we believe one can still
argue that there is a dearth of datasets and research
on multi-party dialogue. 

The impact of training in multi-party settings is not
particularly well understood, as much less prior
work exists in this space compared to the two-party
setting.

\textbf{Perception of an Android Robot in Japan
and Australia: A Cross-Cultural Comparison}
Human perception of robots has been generally shaped by information obtained through social media (e.g. movies, newspaper, internet, etc.) and not by
real interactions with physically present robots.

. In spite of significant research in
HRI, direct contact to a physically present robot is still the exception rather than
the norm. It has been shown, however, that the presence of an embodied robot
plays a crucial role in the way people perceive it [2]. Previous studies also revealed that the expectations and attitude towards robots change based on their
appearance [3]. To accurately evaluate the perception of robots, participants
should ideally be in direct contact with physically present robots [2, 4].

==> notes/reviews.tex <==
- The figures 6 and 7 are too small
TODO: redo the figures

% - can you provide more details on the speech recognition integration 
% TODO: one-liner

% - it is not fully clear is speech to text the main/only input module, and the operator just input metadata and selects the parts of output, not clear also from Fig 2 and 3.
% TODO: one-liner

- The differences between LLMs could be analysed in more detail - since the paper is presented to the scientific community - is there any other difference observed except for the line selection by the curator
TODO: one-liner

% - The technological parts could be described in more detail (e.g. the exact prompts, and how many for modifications (sarcastic, punny, therapy)
% TODO: 

%- it would be nice to have a "lessons learnt section" which would be informative for potential other attempts of AI based improvisation.
% TODO: ignore

% Piotr: include supplement into ICCC and arXiv

